ZIP: An Efficient Zeroth-order Prompt Tuning for Black-box Vision-Language Models

Recent studies have introduced various approaches for prompt-tuning black-box vision-language models, referred to as black-box prompt-tuning (BBPT). While BBPT has demonstrated considerable potential, it is often found that many existing methods require an excessive number of queries (i.e., function evaluations), which poses a significant challenge in real-world scenarios where the number of allowed queries is limited. To tackle this issue, we propose Zeroth-order Intrinsic-dimensional Prompt-tuning (ZIP), a novel approach that enables efficient and robust prompt optimization in a purely black-box setting. The key idea of ZIP is to reduce the problem dimensionality and the variance of zeroth-order gradient estimates, such that the training is done fast with far less queries. We achieve this by re-parameterizing prompts in low-rank representations and designing intrinsic-dimensional clipping of estimated gradients. We evaluate ZIP on 13+ vision-language tasks in standard benchmarks and show that it achieves an average improvement of approximately 6% in few-shot accuracy and 48% in query efficiency compared to the best-performing alternative BBPT methods, establishing a new state of the art. Our ablation analysis further shows that the proposed clipping mechanism is robust and nearly optimal, without the need to manually select the clipping threshold, matching the result of expensive hyperparameter search.

==> figure/fig_abl_clipping_val.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_caltech101.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_oxford_pets.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_flowers.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_food101.pdf}
    \end{subfigure}

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
    
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_fgvc_aircraft.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_sun397.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_dtd.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.245\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_eurosat.pdf}
    \end{subfigure}

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \begin{subfigure}{0.195\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_ucf101.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_svhn.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_resisc45.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_clevr.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.195\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/figures/threshold/validation/clipping_imagenet.pdf}
    \end{subfigure}
    
    \caption{
        Validation curves showing the impact of zeroth-order gradient clipping across various vision-language tasks.
        }
    \label{fig:appendix clipping validation}
\end{figure}
